Benchmarking the Hooke-Jeeves Method, MTS-LS1, and BSrr on the Large-scale BBOB Function Set

This paper investigates the performance of three black-box optimizers exploiting separability on the 24 large-scale BBOB functions, including the Hooke-Jeeves method, MTS-LS1, and BSrr. Although BSrr was not specially designed for large-scale optimization, the results show that BSrr has a state-of-the-art performance on the five separable large-scale BBOB functions. The results show that the asymmetry significantly influences the performance of MTS-LS1. The results also show that the Hooke-Jeeves method performs better than MTS-LS1 on unimodal separable BBOB functions.

==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/ppfigs.tex <==
% Do not modify this file: calls to post-processing software will overwrite any modification.
Legend: {\color{NavyBlue}$\circ$}:BSrr, {\color{Magenta}$\diamondsuit$}:HJ-5, {\color{Orange}$\star$}:HJ-9, {\color{CornflowerBlue}$\triangledown$}:MTSLS1-5, {\color{red}$\varhexagon$}:MTSLS1-9, {\color{YellowGreen}$\triangle$}:LBFGS

==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f001_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f001_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f001_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f001_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f001_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f001_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f002_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f002_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f002_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f002_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f002_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f002_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f003_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f003_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f003_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f003_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f003_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f003_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f004_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f004_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f004_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f004_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f004_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f004_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f005_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f005_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f005_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f005_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f005_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f005_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f006_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f006_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f006_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f006_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f006_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f006_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f007_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f007_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f007_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f007_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f007_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f007_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f008_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f008_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f008_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f008_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f008_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f008_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f009_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f009_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f009_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f009_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f009_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f009_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f010_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f010_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f010_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f010_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f010_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f010_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f011_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f011_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f011_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f011_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f011_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f011_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f012_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f012_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f012_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f012_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f012_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f012_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f013_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f013_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f013_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f013_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f013_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f013_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f014_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f014_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f014_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f014_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f014_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f014_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f015_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f015_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f015_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f015_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f015_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f015_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f016_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f016_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f016_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f016_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f016_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f016_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f017_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f017_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f017_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f017_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f017_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f017_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f018_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f018_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f018_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f018_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f018_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f018_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f019_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f019_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f019_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f019_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f019_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f019_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f020_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f020_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f020_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f020_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f020_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f020_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f021_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f021_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f021_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f021_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f021_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f021_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f022_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f022_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f022_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f022_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f022_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f022_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f023_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f023_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f023_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f023_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f023_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f023_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f024_160D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f024_20D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f024_320D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f024_40D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f024_640D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany-single-functions/pprldmany_f024_80D.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_160D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_160D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_160D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_160D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_160D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_160D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_20D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_20D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_20D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_20D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_20D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_20D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_320D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_320D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_320D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_320D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_320D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_320D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_40D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_40D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_40D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_40D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_40D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_40D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_640D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_640D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_640D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_640D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_640D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_640D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_80D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_80D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_80D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_80D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_80D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> ppdata/BSrr_HJ-5_HJ-9_MTSLS_MTSLS_LBFGS/pprldmany_80D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{BSrr}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{HJ-5}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{HJ-9}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{MTSLS1-5}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{MTSLS1-9}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{LBFGS}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algFperfprof}}}

